PER-ETD: A Polynomially Efficient Emphatic Temporal Difference Learning Method

Emphatic temporal difference (ETD) learning (Sutton et al., 2016) is a successful method to conduct the off-policy value function evaluation with function approximation. Although ETD has been shown to converge asymptotically to a desirable value function, it is well-known that ETD often encounters a large variance so that its sample complexity can increase exponentially fast with the number of iterations. In this work, we propose a new ETD method, called PER-ETD (i.e., PEriodically Restarted-ETD), which restarts and updates the follow-on trace only for a finite period for each iteration of the evaluation parameter. Further, PER-ETD features a design of the logarithmical increase of the restart period with the number of iterations, which guarantees the best trade-off between the variance and bias and keeps both vanishing sublinearly. We show that PER-ETD converges to the same desirable fixed point as ETD, but improves the exponential sample complexity of ETD to be polynomials. Our experiments validate the superior performance of PER-ETD and its advantage over ETD.

==> relatedwork.tex <==
\subsection{Related Works}
\textbf{Finite-sample analysis of TD learning and GTD:} \cite{dalal2018finite} studied the TD($0$) algorithm with i.i.d. samples. They gave both an $\mathcal{O}\left(\frac{1}{T^\sigma}\right)$, $0<\sigma<1$, convergence guarantee in expectation and polynomial convergence rate with high probability. In the meanwhile, \cite{bhandari2018finite} provided an extended analysis which covers both i.i.d. samples case and Markovian samples in a rate of $\tilde{\mathcal{O}}\left(\frac{1}{T}\right)$ convergence in expectation. \cite{lakshminarayanan2018linear} investigated the linear stochastic approximation (SA) with constant stepsize of which TD(0) and GTD could be treated as special cases. They have proven, with i.i.d. samples, linear SA converges with a rate of $\mathcal{O}(\frac{1}{T})$ depending on the variance and $\mathcal{O}(\frac{1}{T^2})$ depending on the initial distance from the fixed point, which match the lower bounds they developed. Recently, \cite{kotsalis2020simple} analyzed the TD learning algorithm with on-policy samples through the lens of generalized monotone variational inequality. They incorporated the TD learning with periodic update and stochastic operator extrapolation technique, which provides huge performance improvement when discounting fact $\gamma$ near to $1$. For the GTD algorithms, \cite{dalal2018finite2,gu2019should} both provided the finite-time analysis of GTD and its variants.

\textbf{Emphatic Temporal Difference Learning:} The emphatic temporal difference learning was originally proposed by \cite{sutton2016emphatic}. In this seminal work, \cite{sutton2016emphatic} introduced the follow-on trace to overcome the distribution mismatch between the behavior policy and the target policy. Later, \cite{yu2015convergence} provided the asymptotic convergence guarantee. \cite{hallak2016generalized} investigated the variance of the follow-on trace and found out that it may has unbounded variance. They proposed a general framework of ETD with a variable decay rate, $\beta\in(0, 1)$, of follow-on trace instead of $\gamma$ in the original design. At the cost of larger approximation error of the fixed point, the variance of follow-on trace is bounded with small $\beta$. \cite{imani2018off} developed a new policy gradient theorem, where the emphatic weighted is used to correct the distribution shift. \cite{zhang2020provably} provided a new variant of ETD, where the emphatic weights are estimated through function approximation.  \cite{van2018deep,jiang2021learning} studied the ETD algorithm with deep neural function class.  %Another line of  \cite{zhang2020provably}
